Strengthening LargeRDFBench for Interoperable Federated SPARQL Evaluation

LargeRDFBench is one of the most comprehensive benchmarks for evaluating federated SPARQL query engines, combining real, interlinked datasets with a rich query suite that has made it a reference point for the community. Evaluations of federated engines are published by comparing engine results against the benchmark's expected results, so those expected results must themselves be reproducible. Moreover, several of its data dumps violate the RDF specifications, so only engines that parse RDF leniently can host them, and its expected results are distributed in an ad hoc format. We identify, categorize and repair these data-quality issues with a reproducible cleaning pipeline, producing standards-conformant serializations of every affected dataset. Furthermore, we re-encode the benchmark's expected results in the W3C SPARQL 1.1 Query Results JSON Format and correct their discrepancies. Every dataset now parses under strict RDF parsers, and the expected results are machine-verifiable through a standard format, extending the benchmark's reach to the full range of conformant engines while staying faithful to the original data. Reproducing the expected results end-to-end with an independent implementation uncovers corruption in the published reference, and discrepancies between our results and the original ones, some not trivial to resolve, others open questions. We further perform a preliminary comparison, not previously explored, of ASK- and COUNT-based source selection in the FedX algorithm. This work strengthens an already valuable community resource by aligning its artifacts with the RDF standards, broadening the set of engines that can be fairly and reproducibly compared. We also raise the question of how the results of federated queries under automatic source selection can be made reproducible.

==> analysis/result-analysis-script/artefact/overview_adhoc/table_overall_ratio_adhoc.tex <==
\begin{table}[t]
	\centering
	\caption{Per configuration: the average \texttt{ASK}/\texttt{COUNT} ratio of
		execution and planning time (mean over the queries that completed in both
		modes), the number of such queries, and the number of failed queries under
		each source-selection strategy.}
	\label{tab:overall-ratio-adhoc}
	\begin{tabular}{lrrrrr}
		\toprule
		Configuration & \multicolumn{2}{c}{\texttt{ASK}/\texttt{COUNT} ratio} & Queries & \multicolumn{2}{c}{Failures} \\
		\cmidrule(lr){2-3}\cmidrule(lr){5-6}
		             & exec. & plan. & used & \texttt{COUNT} & \texttt{ASK} \\
		\midrule
		all-Comunica & 1.8x & 0.9x & 6 & 16 & 17 \\
		mixed        & 2.8x & 2.7x & 5 & 11 & 18 \\
		all-QLever   & 20.8x & 0.8x & 8 & 4 & 16 \\
		\bottomrule
	\end{tabular}
\end{table}


==> analysis/result-analysis-script/makefile <==
RUN           = uv run python
MARIMO        = uv run marimo
NB_DIR        = ./notebooks
ARTEFACT_DIR  = ./artefact

NOTEBOOKS    = overview_adhoc

UTIL_SRC = \
	loaddata.py \
	plots.py \
	tables.py

.PHONY: all sync notebook clean $(NOTEBOOKS)

all: sync $(NOTEBOOKS)

sync:
	uv sync

$(NOTEBOOKS): %: $(NB_DIR)/%.py $(UTIL_SRC)
	$(RUN) $(NB_DIR)/$@.py

notebook:
	@if [ -n "$(nb)" ]; then $(MARIMO) edit $(NB_DIR)/$(nb).py; else $(MARIMO) edit; fi

clean:
	rm -rf $(ARTEFACT_DIR)


==> analysis/result-analysis-script/templates/table_overall_ratio_adhoc.tex <==
\begin{table}[t]
	\centering
	\caption{Per configuration: the average \texttt{ASK}/\texttt{COUNT} ratio of
		execution and planning time (mean over the queries that completed in both
		modes), the number of such queries, and the number of failed queries under
		each source-selection strategy.}
	\label{tab:overall-ratio-adhoc}
	\begin{tabular}{lrrrrr}
		\toprule
		Configuration & \multicolumn{2}{c}{\texttt{ASK}/\texttt{COUNT} ratio} & Queries & \multicolumn{2}{c}{Failures} \\
		\cmidrule(lr){2-3}\cmidrule(lr){5-6}
		             & exec. & plan. & used & \texttt{COUNT} & \texttt{ASK} \\
		\midrule
		all-Comunica & {} & {} & {} & {} & {} \\
		mixed        & {} & {} & {} & {} & {} \\
		all-QLever   & {} & {} & {} & {} & {} \\
		\bottomrule
	\end{tabular}
\end{table}


==> analysis/result-analysis-script/templates/table_qlever_ask_count_adhoc.tex <==
\begin{table}[t]
	\centering
	\caption{Median, minimum and maximum per-query planning and execution time on the
		QLever-hosted federation; the last row is the per-query \texttt{ASK}/\texttt{COUNT}
		ratio (dimensionless).}
	\label{tab:qlever-ask-count-adhoc}
	\begin{tabular}{lrrrrrr}
		\toprule
		                            & \multicolumn{3}{c}{Planning (ms)} & \multicolumn{3}{c}{Execution (s)} \\
		\cmidrule(lr){2-4}\cmidrule(lr){5-7}
		                            & Med & Min & Max & Med & Min & Max \\
		\midrule
		\texttt{ASK}                & {} & {} & {} & {} & {} & {} \\
		\texttt{COUNT}              & {} & {} & {} & {} & {} & {} \\
		\texttt{ASK}/\texttt{COUNT} & {} & {} & {} & {} & {} & {} \\
		\bottomrule
	\end{tabular}
\end{table}


==> makefile <==
SOURCE = main.tex references.bib section/*.tex table/*.tex makefile figure/* \
         analysis/result-analysis-script/artefact/**/*

.PHONY: clean watch

main.pdf: $(SOURCE)
	latexmk -pdf -shell-escape main.tex

watch:
	latexmk -pdf -pvc -shell-escape main.tex

clean:
	rm -f *.log *.aux *.out *.bbl *.blg *.fls *.fdb_latexmk *.synctex.gz \
	      *.bcf *.run.xml *.xmpdata *.xmpi *.abs main.pdf section/*.aux


==> section/preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

TODO.

